First Integrals and symmetries of nonholonomic systems

In nonholonomic mechanics, the presence of constraints in the velocities breaks the well-under\-stood link between symmetries and first integrals of holonomic systems, expressed in Noether's Theorem. However there is a known special class of first integrals of nonholonomic systems generated by vector fields tangent to the group orbits, called {\it horizontal gauge momenta}, that suggest that some version of this link should still hold. In this paper we prove that, under certain conditions on the symmetry Lie group, the (nonholonomic) momentum map is conserved along the nonholonomic dynamics, thus extending Noether Theorem to the nonholonomic framework. Our analysis leads to a constructive method, with fundamental consequences to the integrability of some nonholonomic systems as well as their hamiltonization. We apply our results to three paradigmatic examples: the snakeboard, a solid of revolution rolling without sliding on a plane and a heavy homogeneous ball that rolls without sliding inside a convex surface of revolution. In particular, for the snakeboard we show the existence of a new horizontal gauge momentum that reveals new aspects of its integrability.

==> bibliography.tex <==
{\small
\begin{thebibliography}{99}

%\bibitem{AM}
%\newblock R. Abraham and J.~E. Marsden, 
%\newblock Foundations of Mechanics.
%\newblock Benjamin, Reading 1978.

\bibitem{agostinelli1956}
     \newblock C. Agostinelli,
     \newblock \emph{Nuova forma sintetica delle equazioni del moto di un sistema anolonomo ed esistenza di un integrale lineare nelle velocit\`a.}
     \newblock Boll. Un. Mat. Ital., \textbf{11} (1956), 1--9.

%\bibitem{Arnold}
%\newblock V.I. Arnold,
%\newblock Mathematical Methods of Classical Mechanics. 
%\newblock Graduate Texts in Mathematics {\bf 60} Springer-Verlag, New York,(1989).

\bibitem{AM1997}
\newblock P. Ashwin and I. Melbourne,
\newblock {\it Noncompact drift for relative equilibria and relative periodic orbits.}
\newblock Nonlinearity, {\bf 10} (1997), 595--616.

\bibitem{balseiro2014} 
\newblock P. Balseiro, 
\newblock{\it The Jacobiator of Nonholonomic Systems and the Geometry of Reduced Nonholonomic Brackets.}
\newblock Arch. Ration. Mech. Anal. {\bf 214}, ( 2014), 453--501.

\bibitem{balseiro2017} 
\newblock P. Balseiro, 
\newblock {\it Hamiltonization of Solids of Revolution Through Reduction.}
\newblock  J. Nonlinear Sci. {\bf 27} (2017), 2001--2035.

\bibitem{BalFer2015} 
\newblock P. Balseiro and O.E. Fernandez,
\newblock{\it Reduction of Nonholonomic Systems in Two Stages.} 
\newblock Nonlinearity, Volume 28 (2015) 2873-2912.

\bibitem{BN2011} 
\newblock P. Balseiro and L. Garc\'{i}a-Naranjo, 
\newblock{\it Gauge Transformations, Twisted Poisson Brackets and Hamiltonization of Nonholonomic Systems.} 
\newblock Arch. Ration. Mech. Anal. {\bf 205} (2012), 267--310.

\bibitem{BS2016}
\newblock P. Balseiro and N. Sansonetto,
\newblock{\it A Geometric Characterization of Certain First Integrals for Nonholonomic Systems with Symmetries.}
\newblock SIGMA {\bf 12} (2016), 018, 14pages.

\bibitem{BalYapu19} 
\newblock P. Balseiro and L.P. Yapu. 
\newblock{\it Conserved quantities and hamiltonization of nonholonomic systems.} 

%\bibitem{BC}
%\newblock L.M. Bates and R.H. Cushman, 
%\newblock {\em What is a completely integrable nonholonomic dynamical system?}
%\newblock Rep. Math. Phys. {\bf44} (1999), 29--35.

%\bibitem{bluebook}
%\newblock L.M. Bates and R.H. Cushman, 
%\newblock Global aspects of classical integrable systems. Second edition.
%\newblock Birkh\"auser Verlag, Basel, 1997.

\bibitem{BGM96}
\newblock L.M.~Bates, H.~Graumann and C.~MacDonnell,
\newblock {\it Examples of gauge conservation laws in nonholonomic systems.}
\newblock \emph{Rep. Math. Phys.}, \textbf{37} (1996), 295--308.

\bibitem{BS93}
\newblock L.M. Bates and J. \'Sniatycki, 
\newblock {\em Nonholonomic reduction.}
\newblock Rep. Math. Phys. {\bf32} (1993), 99--115.

%\bibitem{BS2016} 
%L. Bates and J. Sniatycki, 
%{\it Not quite hamiltonian reduction, ....}    

%\bibitem{benenti2007} 
%\newblock S. Benenti,
%\newblock \emph{A 'User-Friendly' Approach to the Dynamical Equations of Non-Holonomic Systems.}
%\newblock SIGMA, \textbf{3} (2007), 33 pp.

%\bibitem{benenti2008} 
%\newblock S. Benenti,
%\newblock \emph{A general method for writing the dynamical equations of	nonholonomic systems with ideal constraints.}
%\newblock{Regul. Chaotic Dyn., \textbf{13} (2008), 283--315.}

\bibitem{Bloch}
\newblock A.M. Bloch, 
\newblock Nonholonomic Mechanics and Controls. 2nd Edition.
\newblock Interdisciplinary Applied Mathematics {\bf 24}, Systems and Control.
(Springer--Verlag, New York, 2015).

\bibitem{BKMM}
     \newblock A.M. Bloch, P.S. Krishnaprasad, J.E. Marsden, R.M. Murray,
     \newblock {\it Nonholonomic mechanical systems with symmetry.}
     \newblock Arch. Rational Mech. Anal. \textbf{136}  (1996), 21--99.

%\bibitem{BMZ}
%     \newblock A.M. Bloch, J.E. Marsden and D.V. Zenkov,
%     \newblock \emph{Quasivelocities and symmetries in non--holonomic systems.}
%     \newblock Dynamical Systems \textbf{24} No. 2 (2009), 187--222.

\bibitem{bogoyavlenskij} % (MR1643501) [10.1007/s002200050412]
\newblock O. I. Bogoyavlenskij,
\newblock {\it Extended integrability and bi-{H}amiltonian systems.}
\newblock Comm. Math. Phys., \textbf{196} (1998), 19--51.

\bibitem{BKK2015} 
\newblock{A.V. Bolsinov, A.A. Kilin, and A.O. Kazakov,}
\newblock{\it Monodromy as an obstruction to Hamiltonization: pro or contra?} 
\newblock{J. Geom. Phys. {\bf 87} (2015), 61--75.}

%\bibitem{BBM2011} 
%\newblock A.V. Bolsinov, A.V. Borisov, and I.S. Mamaev
%\newblock{\it Hamiltonization of Non-Holonomic Systems in the Neighborhood of Invariant Manifolds.}
%\newblock{Regul Chaotic Dyn., {\bf 16} (2011), 443--464.} 

%\bibitem{BM2002} 
%\newblock A.V. Borisov and I.S. Mamaev,
%\newblock {\it The rolling motion of a rigid body on a plane and a sphere, Hierarchy of dynamics.} 
%\newblock Regul. Chaotic Dyn., {\bf 7}  (2002), 201--219. 

\bibitem{BorisovMamaev2001} 
\newblock A.~V. Borisov and  I.~S. Mamaev,  
\newblock {\it Chaplygin's ball rolling problem is Hamiltonian.}
\newblock  Math. Notes, {\bf 70} (2001), 793--795.

\bibitem{BMK2002} 
\newblock A.V. Borisov,  I.S. Mamaev and A.A. Kilin,
\newblock {\it Rolling of a ball on a surface. New integrals and hierarchy of dynamics.} 
\newblock Regul. Chaotic Dyn., {\bf 7}  (2002), 177--200. 

%\bibitem{BorisovMamaev2008} 
%\newblock A.~V. Borisov and  I.~S. Mamaev,  
%\newblock {\it Conservation laws, Hierarchy of dynamics and explicit integration of nonholopnomic systems.}
%\newblock Regul. Chaotic Dyn., {\bf 13}  (2008), 443--489. 

%\bibitem{Bullo-Lewis}
%\newblock F. Bullo and A.D. Lewis, 
%\newblock{\em Geometric control of mechanical systems. Modeling, analysis, and design for simple mechanical control systems.} 
%\newblock Texts in Applied Mathematics {\bf 49} (Springer-Verlag, New York, 2005).

%\bibitem{byers1}
%N. Byers, {\em The life and time of Emmy Noether: Contributions of
%Emmy Noether to particle physics}. arXiv:hep-th/9411110v2 (1994)
%
%\bibitem{byers2}
%N. Byers, {\em E. Noether's discovery of the deep connection between
%symmetries and conservation laws.} In {\em The heritage of Emmy Noether
%(Ramat-Gan, 1996)}, Israel Math. Conf. Proc. {\bf 12}, 67--81, Bar-Ilan
%Univ., Ramat Gan, 1999.

\bibitem{CdLdDM}
\newblock F. Cantrijn, M. de Leon, M. de Diego and J. Marrero,
\newblock \emph{Reduction of nonholonomic mechanical systems with symmetries},
\newblock Rep. Math. Phys. \textbf{42} (1998), 25--45.

\bibitem{CCdLdD}
\newblock F. Cantrijn, J. Cort\'es, M. de Leon and M. de Diego,
\newblock {\it On the geometry of generalized Chaplygin systems},
\newblock Math. Proc. Cambridge Phil. Soc. {\bf 132} (2002), 323--351.

\bibitem{chapsphere} 
\newblock S.~A. Chaplygin,  
\newblock {\it On a ball's rolling on a horizontal plane. }
\newblock Regul.  Chaotic Dyn., {\bf 7} (2002), 131--148; original paper in Mathematical Collection of the Moscow
Mathematical Society, {\bf 24} (1903), 139--168.

\bibitem{cortes}
\newblock J. Cort\'es Monforte, 
\newblock Geometric, control and numerical aspects of nonholonomic systems.
\newblock Lecture Notes in Mathematics {\bf 1793} (Springer-Verlag, Berlin, 2002).

\bibitem{cushman1998} 
\newblock R.Cushman, 
\newblock {\it Routh's sphere.} 
\newblock Rep. on Math. Phys. {\bf 42} (1998), 42--70.

\bibitem{CKSB}
\newblock R. Cushman, D. Kemppeinen, J. \'Sniatycki and L. M.~Bates,
\newblock {\it Geometry of nonholonomic constraints.}
\newblock Rep. Math. Phys., \textbf{36} (1995), 275--286.

%\bibitem{CB}
%\newblock R.H. Cushman and L.M. Bates,
%\newblock Global Aspects of Classical Integrable Systems.
%\newblock Birkh\"auser/Springer, Basel, 2015.

%\bibitem{CD2001}
%\newblock R.H. Cushman and J.J. Duistermaat,
%\newblock {\it Non--Hamiltonian Monodromy}.
%\newblock J. Differential Equations {\bf 172} (2001), 42--58.

\bibitem{CDS}
\newblock R. Cushman, J.J. Duistermaat and J. \'Sniatycki,
\newblock Geometry of Nonholonomically Constrained Systems. 
\newblock Advanced Series in Nonlinear Dynamics {\bf 26}, Singapore: World Scientific, 2010.

%\bibitem{CS2007}
%\newblock R. Cushman and J. \'Sniatycki, 
%\newblock {\it Non--holonomic reduction of symmetries, constraints, and integrability.}
%\newblock Regul. Chaotic Dyn. {\bf 12} (2007), 615--621.

%\bibitem{dLCdDM} 
%\newblock M. de Leon, J. Cortes, M. de Diego and S. Mart\'{i}nez, 
%\newblock {\it Introduction to Mechanics and Symmetry.} 
%\newblock In: I. Bajo and E. Sanmartin (eds), {\it Recent Advances in Lie Theory}.
%Research and Exposition in Mathematics Series {\bf 25}, 305-332 (Heldermann Verlag, 2002),
%
%\bibitem{dLMMdD1997}
%\newblock M. de Le\'on, J.C. Marrero and D. Mart\'{\i}n de Diego,
%\newblock {\it Mechanical systems with nonlinear constraints.}
%\newblock Int. J. Th. Phys. \textbf{36} (1997), 979--995.

%\bibitem{DD1987}
%\newblock P. Dazord and T. Delzant,
%\newblock{\it Le probleme general des variables actions-angles.}
%\newblock J. Diff. Geom. {\bf 26} (1987), 223--251.

%\bibitem{duistermaat1980}
%\newblock J.J. Duistermaat, 
%\newblock {\it On global action-angle coordinates.}
%\newblock Comm. Pure Appl. Math. {\bf 33} (1980), 687-706.

\bibitem{duistermaat2004}
\newblock J.J. Duistermaat, 
\newblock {\it Chaplygin's sphere.} 
\newblock arXiv:math/0409019 (2004).


%\bibitem{fasso98}
%\newblock F. Fass\`o,
%\newblock {\it Quasi--periodicity of motions and complete integrability of Hamiltonian systems.}
%\newblock Ergodic Theory and Dynamical Systems {\bf 18} (1998), 1349--1362.

%\bibitem{fasso}
%\newblock F. Fass\`o,
%\newblock {\it Notes on Finite Dimensional Integrable Hamiltonian Systems.}
%\newblock Unpublished notes available at http://www.math.unipd.it/~fasso/research/papers/sc.pdf

\bibitem{FG2002}
\newblock F. Fass{\` o} and A. Giacobbe,
\newblock {\it Geometric structure of "broadly integrable" Hamiltonian systems.}
\newblock J. Geom. Phys. \textbf{44} (2002), 156--170.

\bibitem{FG2007}
\newblock F. Fass\`o and A. Giacobbe, 
\newblock{\it Geometry of Invariant Tori of Certain Integrable Systems with Symmetry and an Application
to a Nonholonomic System.}
\newblock SIGMA {\bf 3} (2008), 051.

\bibitem{FGS2005}
\newblock F. Fass{\` o}, A. Giacobbe and N. Sansonetto,
\newblock {\it Periodic flows, rank--two Poisson structures, and Nonholonomic systems.}
\newblock Reg. Ch. Dyn. \textbf{10} (2005), 267--284.

\bibitem{FGS2008}
\newblock F. Fass{\` o}, A. Giacobbe and N. Sansonetto,
\newblock \emph{Gauge conservation laws and the momentum equation in nonholonomic mechanics.}
\newblock Rep. Math. Phys. \textbf{62} No. 3 (2008), 345--367.

\bibitem{FGS2009}
\newblock F. Fass{\` o}, A. Giacobbe, N. Sansonetto,
\newblock \emph{On the number of weakly Noetherian constants of motion of nonholonomic systems.}
\newblock J. Geom. Mech. \textbf{1} (2009) 389--416.
     
\bibitem{FS2010}
\newblock F. Fass{\` o} and N. Sansonetto,
\newblock {\it An Elemental Overview of the Nonholonomic Noether Theorem.}
\newblock Int. J. Geom. Methods Mod. Phys. {\bf 6} (2010), 1343--1355.

\bibitem{FGS2012}
\newblock F. Fass{\` o}, A. Giacobbe, N. Sansonetto,
\newblock {\it Linear weakly Noetherian constants of motion are horizontal gauge momenta.}
\newblock J. Geom. Mech. \textbf{4} (2012) 129--136.

\bibitem{FRS2007}
\newblock F. Fass{\` o}, A. Ramos, N. Sansonetto,
\newblock {\it The reaction-annihilator distribution and the nonholonomic Noether theorem for lifted actions.}
\newblock Reg. Ch. Dyn. \textbf{12} (2007), 579--588.

\bibitem{FPZ2020}
\newblock F. Fass\`o. S. Passarella, and M. Zoppello, 
\newblock{\it Control of locomotion systems and dynamics in relative periodic orbits.}
\newblock To appear in J. Geom. Mech. doi:10.3934/jgm.2020022.

\bibitem{fedorov} %(MR1720911)
\newblock Y. N. Fedorov,
\newblock {Systems with an invariant measure on Lie groups},
\newblock In \emph{Hamiltonian systems with three or more degrees of freedom (S'Agar\`o, 1995)}, 350--356, NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci., 533 Kluwer, Dordrecht, 1999.

\bibitem{field1990} 
M.J. Field, 
{\it Equivariant dynamical systems.} 
Trans. Am. Math. Soc. {\bf 259} (1990), 185--205.  

%\bibitem{field1991}
%\newblock M. Field,
%\newblock {\it Local structure of equivariant dynamics, in Singularity Theory and Its Applications, Part II .}
%\newblock Lecture Notes in Math., {\bf 1463} Springer--Berlin (1991), 142--166.

%\bibitem{Gallier} 
%\newblock J.~Gallier,
%\newblock Notes on Differential Geometry and Lie Groups. 
%\newblock Springer, Geometry and Computing Series, 2020.

\bibitem{GN2008}  
\newblock L. Garcia-Naranjo
\newblock \emph{Reduction of  almost Poisson brackets and hamiltonization of the Chaplygin sphere.}
\newblock  Disc. and Cont. Dyn. Syst. Series S, {\bf 3}, (2010), %no. 1, 
37--60.

\bibitem{GNMontaldi}  
\newblock L.C. Garc\'ia-Naranjo and J. Montaldi
\newblock \emph{Gauge momenta as Casimir functions of nonholonomic systems.}
\newblock  Arch Rational Mech Anal (2018), 228 (2), pp 563-602

\bibitem{hermans}
\newblock J. Hermans,
\newblock {\it A symmetric sphere rolling on a surface.}
\newblock Nonlinearity, {\bf 8} (1995), 493--515.

\bibitem{IdLMM} 
\newblock A. Ibort, M. de Le\'on, J. C. Marrero, D. Mart\'\i n de Diego
\newblock {\it Dirac brackets in constrained dynamics.}
\newblock Fortschritte der Physik, Vol.47 (1999), 459--492.


\bibitem{iliev1}
\newblock Il. Iliev and Khr. Semerdzhiev,
\newblock \emph{Relations between the first integrals of a nonholonomic mechanical system and of the corresponding system freed of constraints.}
\newblock J. Appl. Math. Mech. \textbf{36}  (1972), 381--388.

\bibitem{iliev2}
\newblock Il. Iliev,
\newblock \emph{On first integrals of a nonholonomic mechanical system.}
\newblock J. Appl. Math. Mech. \textbf{39}  (1975), 147--150.

%\bibitem{jovanovic}
%\newblock B. Jovanovic, 
%\newblock {\it Symmetries and Integrability.} 
%\newblock Publications de l'Institut Math\'ematique (Beograd), {\bf 84} (2008), 1--36.

%\bibitem{koiller}
%\newblock J. Koiller,
%\newblock \emph{Reduction of some classical nonholonomic systems with symmetry},
%\newblock Arch. Rat. Mech. An. {\bf 118} (1992), 113--138.

%\bibitem{kosmann1985}
%\newblock Y. Kosmann-Schwarzbach, 
%\newblock {\em Sur les th\'eor\`emes de Noether.} 
%\newblock G\'eom\'etrie et physique (Marseille-Luminy, 1985). Travaux en Cours {\bf 21}, 147--160 (Hermann, Paris, 1987).
%
%\bibitem{kosmann2006}
%\newblock Y. Kosmann-Schwarzbach, 
%\newblock {\em Les th\'eor\`emes de Noether. Invariance et lois de conservation au XX$\sp{\rm e}$ si\`ecle.}
%\newblock {\'Editions de l'\'Ecole Polytechnique} (Palaiseau, 2006).

%\bibitem{KK1978}
%\newblock V.V. Kozlov and N.N. Kolesnikov, 
%\newblock {\it On theorems of dynamics.}  
%\newblock J. Appl. Math. Mech. {\bf 42 } (1978), 28--33. 

\bibitem{krupa}
M. Krupa,
{\it Bifurcations of relative equilibria.} 
SIAM J. Math. Anal. {\bf 21} (1990), 1453--86.

%\bibitem{LM94}
%\newblock A. Lewis and R.M. Murray,
%\newblock {\it Variational principles in constrained systems: theory and experiments.}
%\newblock  Intern. J. Nonlinear Mech {\bf 30} (1994), 793--815.


\bibitem{marle95}
\newblock C.-M. Marle,
\newblock {\it Reduction of constrained mechanical systems and stability of relative equilibria.}
\newblock Comm. Math. Phys. {\bf 174} (1995), 295--318.

\bibitem{Marle98}
\newblock C.-M. Marle,
\newblock {\it Various approaches to conservative and nonconservative nonholonomic systems.}
\newblock Rep. Math. Phys. {\bf 42} (1998), 211--229.

\bibitem{marle2001}
\newblock C.-M. Marle,
\newblock \emph{On symmetries and constants of motion in Hamiltonian systems with nonholonomic constraints},
\newblock  In ``Classical and quantum integrability'' (Warsaw, 2001), 223--242, Banach Center Publ.~{\bf 59} 2001, Polish Acad. Sci. Warsaw (2003),  223--242

\bibitem{MarsdenRatiuBook}
\newblock J.E. Marsden and T.S. Ratiu,
\newblock Introduction to Mechanics and Symmetry, 2nd ed.
\newblock Texts in Appl. Math. New York, Springer, {\bf 17}, 1999.

\bibitem{milnor1976}
\newblock J. Milnor,
\newblock \emph{Curvatures of Left Invariant Metrics on Lie Groups}.
\newblock  Advances in Mathematics \textbf{21} (1976), 293--329.

%\bibitem{MF1978}
%\newblock A.S. Mischenko and A. T. Fomenko,
%\newblock {\it Generalized Liouville method of integration of Hamiltonian systems.}
%\newblock Funct. Anal. Appl. \textbf{12} (1978), 113--121.

\bibitem{Naber}
\newblock G.L. Naber,
\newblock Topology, Geometry and Gauge Fields. Applied Mathematical Sciences, {\bf 141}.
\newblock  Springer, Heidelberg, 1991.

\bibitem{Nash}
\newblock Ch. Nash,
\newblock Differential Topology and Quantum Field Theory.
\newblock Academic Press, New York, 1991.

\bibitem{NF}
\newblock Ju.I. Neimark and N.A. Fufaev,
\newblock Dynamics of Nonholonomic Systems. 
\newblock Translations of Mathematical Monographs {\bf 33} (AMS, Providence, 1972).

%\bibitem{nekhoroshev}
%\newblock N. N. Nekhoroshev,
%\newblock {\it Action--angle variables and their generalizations.}
%\newblock Trans. Moskow Math. Soc. \textbf{26} (1972), 181--198.

%\bibitem{noether}
%\newblock E. Noether, 
%\newblock {\em  Invarianten beliebiger Differentialausdr\"ucke.}
%\newblock Nachr. Akad. Wiss. G\"ottingen Math.-Phys. Kl. II 1918, 235--257. English translation: {\em Invariant variation problems}, Transport Theory Statist. Phys. {\bf 1}  (1971), 186--207.

%\bibitem{OR}
%\newblock J.P. Ortega and T.S. Ratiu,
%\newblock Momentum maps and Hamiltonian reduction.
%\newblock Birkh\"auser, Boston 2004.

\bibitem{OLMB}
\newblock J. Ostrowski, A. Lewis, R. Murray and J. Burdick
\newblock {\it Nonholonomic mechanics and locomotion: the snakeboard example.}
\newblock Proceedings of the 1994 IEEE International Conference on Robotics and Automation.


%\bibitem{parasiuk1}
%\newblock I.O. Parasiuk, 
%\newblock {\it Co--isotropic invariant tori of Hamiltonian systems in the quasiclassival theory of the motion of a conduction electron.} 
%\newblock Ukrainian Math J. {\bf 42} (1990), 308--312.
%
%\bibitem{parasiuk2}
%\newblock I.O. Parasiuk, 
%\newblock {\it Variables of action--angle type on symplectic manifolds stratifies by coisotropic tori.} 
%\newblock Ukrainian Math J. {\bf 45} (1993), 85--93.
%
%\bibitem{parasiuk3}
%\newblock I.O. Parasiuk, 
%\newblock {\it Reduction and coisotroopic invariant tori of Hamiltonian systems with non--Poisson commutative symmetries. II.} 
%\newblock Ukrainian Math J. {\bf 46} (1994), 991--1002.

%\bibitem{Pars}
%\newblock L. Pars, 
%\newblock A Treatise on Analytical Dynamics. 
%\newblock Heinemann, New York, 1965.

\bibitem{Routh}
\newblock E.J. Routh, 
\newblock Treatise on the Dynamics of a System of Rigid Bodies (Advanced Part). 
\newblock Dover, New York, 1955.

\bibitem{RS}
\newblock G. Rudolf and M. Schmdt, 
\newblock {Differential Geometry and Mathematical Physics. Part 2.} 
\newblock Theoretical and Mathematical Physics Series, 2017.

\bibitem{sansonetto}
\newblock N. Sansonetto, 
\newblock {First integrals in nonholonomic systems.} 
\newblock Ph.D. thesis, Universit\`a degli Studi di Padova.

\bibitem{SVN}
\newblock D. Sepe and S. Vu Ngoc, 
\newblock {Integrable systems, symmetries, and quantization.} 
\newblock Lett. Math. Phys. {\bf 108} (2018), 499--571.

\bibitem{SeveraWeinstein} 
\newblock P. \v{S}evera, A. Weinstein, 
\newblock {\it Poisson Geometry with a 3-form Background.}
\newblock Progress of Theoretical Physics, Vol. 144 (2001), 145-154.

\bibitem{Sniatycki98}
\newblock J. Sniatycki,
\newblock {\it Nonholonomic Noether theorem and reduction of symmetries.}
\newblock Rep. Math. Phys. \textbf{42} (1998), 5-23.

\bibitem{ShaftMashke}
\newblock A. Van der Shaft and B.M. Mashke, 
\newblock{\it On the Hamiltonian formulation of nonholonomic mechanical systems.}
\newblock Rep. Math. Phys. {\bf 34} (1994), 225-233. 

%\bibitem{winternitz2004}
%\newblock P. Winternitz, 
%\newblock{\it Superintegrable Systems in Classical and Quantum Mechanics.}
%\newblock{In In: Shabat A.B., Gonz\'alez-L\'opez A., Ma\~nas M., Mart\'{i}nez Alonso L., Rodr\'{i}guez M.A. 
%(eds) New Trends in Integrability and Partial Solvability. NATO Science Series 
%(Series II: Mathematics, Physics and Chemistry), vol 132. Springer, Dordrecht.}

\bibitem{zenkov1995}
\newblock D.V. Zenkov, 
\newblock{\it The geometry of the Routh problem.}
\newblock J. Nonlinear Sci. {\bf 5} (1995), 503-519. 

\bibitem{zenkov2003}
\newblock D.V. Zenkov,
\newblock \emph{Linear conservation laws of nonholonomic systems with symmetry.}
\newblock In ``Dynamical systems and differential equations'' (Wilmington, NC, 2002),  
Discrete Contin. Dyn. Syst. suppl. (2003), 967--976.

%\bibitem{zung2006}
%\newblock N,T. Zung,
%\newblock {\it Torus action and integrable systems, in Topological Methods in the Theory of Integrable Systems.}
%\newblock  Editors A.V. Bolsinov, A.T. Fomenko and A.A. Oshemkov, Cambridge Scientific Publications  (2006), 289-328, math.DS/0407455.

\bibitem{zung2016}
\newblock N.T. Zung,
\newblock {\it Geometry of Integrable non--Hamiltonian Systems, Geometry and Dynamics of Integrable Systems. Advanced Courses in Mathematics, CRM Barcelona.}
\newblock Editors V. Matveev and E. Miranda, Birkh\"auser (2016), 85-135.

%\bibitem{zung2017}
%\newblock N,T. Zung,
%\newblock{\it A conceptual approach to the problem of action-angle variables.}
%\newblock arXiv:1706.08859

%\bibitem{zung-minh2013}
%\newblock N.T. Zung, N.V. Minh, 
%\newblock{\it Geometry of integrable dynamical systems on 2-dimensional surfaces.} 
%\newblock Acta Math. Vietnam. {\bf 38} (2013), 79-106.

\end{thebibliography}
}

